Hollywood's misrepresentation of death: A comparison of overall and by-gender mortality causes in film and the real world

The common phrase 'representation matters' asserts that media has a measurable and important impact on civic society's perception of self and others. The representation of health in media, in particular, may reflect and perpetuate a society's disease burden. Here, for the top 10 major causes of death in the United States, we examine how cinematic representation of overall and by-gender mortality diverges from reality. Using crowd-sourced data on film deaths from Cinemorgue Wiki, we employ natural language processing (NLP) techniques to analyze shifts in representation of deaths in movies versus the 2021 National Vital Statistic Survey (NVSS) top ten mortality causes. Overall, movies strongly overrepresent suicide and, to a lesser degree, accidents. In terms of gender, movies overrepresent men and underrepresent women for nearly every major mortality cause, including heart disease and cerebrovascular disease. The two exceptions for which women are overrepresented are suicide and accidents. We discuss the implications of under- and over-representing causes of death overall and by gender, as well as areas of future research.

==> correspondence/general.settings.tex <==
\usepackage{graphicx}
\usepackage{url}
\usepackage{hyperref}

\usepackage{marvosym}

\usepackage[svgnames]{xcolor}
\definecolor{lightgrey}{rgb}{0.7,0.7,0.7}
\definecolor{grey}{rgb}{0.5,0.5,0.5}


\setlength{\oddsidemargin}{20pt}
\setlength{\topmargin}{-20pt}
\setlength{\textwidth}{5in}
\setlength{\textheight}{600pt}

\setlength{\parindent}{0pt}
\setlength{\parskip}{10pt}

\pagestyle{plain}

\renewcommand{\baselinestretch}{1.1}

\newcommand{\etal}{\textit{et al.}}


==> film-deaths-manuscript.settings.tex <==
\newcommand{\filenamebase}{film-deaths}


==> film-deaths.author.tex <==
\author{
\firstname{Other}
\surname{Humans}
}
\email{us@humans.edu}

\affiliation{
  The Earth
}

\author{
\firstname{Captain}
\surname{Bananapants}
}
\email{banana@pants.edu}

\affiliation{
  Elsewhere.
}


==> film-deaths.biblio.tex <==
\bibliography{\filenamebase}


==> film-deaths.changelog.tex <==
%% for arXivs of the various stripes

\todo{Notes on what has changed}
\todo{complete: Check Wenger reference; name has null, null}
\\
      \todo{Increase font size in figure to be close to be close to but smaller than the font size of main text (more like Figure 3)}\\
      \todo{Add more to caption with view that this is all someone might read.}\\
      \todo{Remove legend.}\\
      \todo{Add ``identity line'' along dashed line, rotating text}\\
      \todo{Horizontal axis label: ``Number of recorded deaths in the US, 2021''}\\
      \todo{Vertical axis label: ``Number of film deaths''}\\
      \todo{Bottom axis should come out of zero point which means annotations need to be higher up}\\
      \todo{How does this graph look on a log scale?}\\
      \todo{Make this figure a PDF}

      For Figure 3:\\
\todo{Re-order from most misrepresented to least misrepresented; use same ordering Table 3}
\todo{Remove legend}\\
\todo{Add ``50/50'' at the very top of the dashed line}\\
\todo{Add tick labels to all bottom axes (not just the last one); use minor gray scale to background them a little}\\
\todo{Remove tick marks on vertical axes}\\
\todo{Add colon after each mortality cause label (will make it more clear that these labels are titles connected to the bars below}\\
\todo{Shrink the gap between bar plots a little}\\
\todo{Make this figure a PDF}

\\
    \todo{Note: Changed $\chi^{2}$ and
    $p$-values to 2 significant figures}

    \todo{Because ranking top 10 overall, then this can be removed: ``Other'' causes of death are all deaths not captured in the categories above (does not include chronic liver disease and suicide)}

      \todo{Re-order as Total count, Female count, Female \%, Male count, Male \%; have done for the first two}\\
  \todo{List ranks for female and male in parentheses as suggested in table}\\
  \todo{3 sig figs for percentages}\\
  \todo{add commas to integers}

  \todo{Suggest removing; then tables/figures in main text will be all strong}
  \todo{Or: remove and integrate numbers/percentages into Figure 2 (there is plenty of room)}
  \todo{Or: Make this into a simple LaTeX table}\\
  \todo{Note: All figures should be stand alone pdfs}
  \todo{Possibly put in appendix}

  \todo{Emphasize results for (1) overall disparity in death by type and (2) disparity between genders}

\todo{*,**,*** used for significance; change to another symbol}

\todo{Note: leave blank lines only between paragraphs; this is all LaTeX needs}

\todo{Note: leave at least one blank line before and after each section heading}

\todo{Note: put a tilde before cite and ref commands to prevent awkward line breaks}

\todo{Note: em dash is three hyphens; connect words around em dash}

\todo{Make captions succinctly self-sufficient}

\todo{Notes for captions just go into captions}

\todo{Note: the $p$ in $p$-value is a `math p'}

\todo{All figures have to be separate files (ideally pdfs); no tikz in paper document}

\todo{Add commas to all numbers in the 1000s and above}

\todo{3 sig figs is generally good}

\todo{Write equations, tables, etc. in LaTeX using vertical space; linebreak; easy to read in LaTeX, easier to edit}

\todo{subsections and subsections: need to be at least 2}


==> film-deaths.contributions.tex <==
Who did what.


==> film-deaths.keywords.tex <==
%% one per line, comma separated

mortality,
gender equity,
women's health,
film studies,
representation,




==> film-deaths.methods.tex <==
\section{Methods}
\label{sec:papertag.methods}






==> film-deaths.nutshell.tex <==
\todo{Write a 1--3 sentence nutshell (logline)}


